On Parameterized Complexity of Binary Networked Public Goods Game

In the Binary Networked Public Goods game, every player needs to decide if she participates in a public project whose utility is shared equally by the community. We study the problem of deciding if there exists a pure strategy Nash equilibrium (PSNE) in such games. The problem is already known to be NP-complete. We provide fine-grained analysis of this problem under the lens of parameterized complexity theory. We consider various natural graph parameters and show either W[1]-hardness or exhibit an FPT algorithm. We finally exhibit some special graph classes, for example path, cycle, bi-clique, complete graph, etc., which always have a PSNE if the utility function of the players are fully homogeneous.

==> best.tex <==
\section{Finding Utility functions using best responses}
\begin{observation}
Given the best response functions $\beta_v$ of each player $v$, we can find the Utility functions which replicate the best responses.
\end{observation}
Let the utility function of $v$ be $U_{v}(x_v,n_v)=g_v(x_v+n_v)-c_v\cdot x_v$. Let $c_v$ be a constant greater than 1. Let $g_v(0)=C$ where $C$ is greater than 0. Now we define $g_v(.)$ recursively in the following way:\\
 $g_v(x)= \left\{ \begin{array}{rcl}
g_v(x-1)+c_v-1 & \mbox{if} & 1\notin\beta_v(x-1)  \\ 
g_v(x-1)+c_v+1 & \mbox{if} & 0\notin\beta_v(x-1)  \\ 
g_v(x-1)+c_v & \mbox{if} & 0,1 \in \beta_v(x-1)  \\ 
\end{array}\right.$\\
In the above recursive definition, $x$ belongs to [d(v)+1], where $d(v)$ is the degree of $v$.
Now we show that if $n_v=x-1$ and the player $v$ plays 1 then $1\in\beta_v(x-1)$ and if the player $v$ plays 0 then $0\in \beta_v(x-1)$.  If a player plays 1 then $U_v(1,x-1)\geq U_v(0,x-1)$ otherwise it would deviate to 0. This implies $g_v(x)-c_v\geq g_v(x-1)$. This happens iff $g_v(x$) is either $g_v(x-1)+c_v+1$ or $ g_v(x-1)+c_v$ and in either case $1\in \beta_v(x-1)$. Similarly if a player plays 0 then $U_v(1,x-1)\leq U_v(0,x-1)$ otherwise it would deviate to 1. This implies $g_v(x)-c_v\leq g_v(x-1)$. This happens iff $g_v(x)$ is either $g_v(x-1)+c_v-1$ or  $g_v(x-1)+c_v$ and in either case $0\in \beta_v(x-1)$.

==> bugs.tex <==
\section{Heterogeneous BNPG game on a complete graph}\label{prop2:fix}
Let us have a complete graph $G(V,E)$. $\forall k>0$, let $\mathcal{S}(k)=\{i|c_i\geq \Delta g_i(k),\forall i\in V\}$ and let $\mathcal{R}(k)=\{i|c_i\leq \Delta g_i(k-1),\forall i\in V\}$. Then we have the following proposition:
\begin{proposition}
In a complete graph $G(V,E)$ there exists a PSNE where all the responses are not 0 if and only if $\exists 0< k\leq n:|\mathcal{R}(k)|\geq k$, $|\mathcal{S}(k)|\geq |V|-k$ and $|\mathcal{S}(k)\setminus \mathcal{R}(k)|=|V\setminus \mathcal{R}(k)|$
\end{proposition}
\begin{proof}
If there exists a PSNE with $k>0$ responses as 1, then we have a set $\mathcal{K}_1$ of at least $k$ players  such that $\forall v\in \mathcal{K}_1$, $c_v\leq \Delta g_v(k-1)$. So $|\mathcal{R}(k)|\geq k$. Since $|V|-k$ players have their responses as 0 in the PSNE, it means that we have a set $\mathcal{K}_2$ of at least $|V|-k$ players such that $\forall v\in \mathcal{K}_2$, $c_v\geq \Delta g_v(k)$. So $|\mathcal{S}(k)|\geq |V|-k$. Also, for any player $v$ which doesn't belong to $\mathcal{R}(k)$, it's response is 0 which implies that $v\in \mathcal{S}(k)$. And $\mathcal{S}(k)\setminus \mathcal{R}(k)\subseteq V\setminus \mathcal{R}(k)$. Hence, we also have $|\mathcal{S}(k)\setminus \mathcal{R}(k)|=|V\setminus \mathcal{R}(k)|$.
\\ \\
In the other direction, let us assume that $\exists 0< k\leq n:|\mathcal{R}(k)|\geq k$, $|\mathcal{S}(k)|\geq |V|-k$ and $|\mathcal{S}(k)\setminus \mathcal{R}(k)|=|V\setminus \mathcal{R}(k)|$. Let the response of all the players in $V\setminus \mathcal{R}(k)$ be 0 (all such players belong to $\mathcal{S}(k)$ otherwise $|V\setminus \mathcal{R}(k)|$ would have been greater than $|\mathcal{S}(k)\setminus \mathcal{R}(k)|$) . Choose $|V|-k-|V\setminus \mathcal{R}(k)|$ players from $\mathcal{R}(k)\cap\mathcal{S}(k)$ and make their response as 0. Note that this is possible as $|\RR(k)\cap\SS(k)|=|\SS(k)|-|V\setminus\RR(k)|\geq|V|-k-|V\setminus \mathcal{R}(k)|\geq 0$ .Make responses of rest of the $k$ players as 1. Clearly players whose responses are 1 won't deviate as they belong to $\mathcal{R}(k)$ and players whose response are 0 won't deviate as they belong to $\mathcal{S}(k)$.

This concludes the proof of this proposition.
\end{proof}

\begin{proof}[Proof of \Cref{obs:complete}]
We now propose the following Algorithm to check whether there is PSNE or not where exactly $k$ players play $1$. First if $k=0$ and $|\mathcal{S}(0)|=n$, we have a PSNE where all the responses are 0 else we don't have such a PSNE. Otherwise, for a $k$ greater than 0 and less than or equal to $n$, we check whether the conditions $|\mathcal{R}(k)|\geq k$, $|\mathcal{S}(k)|\geq |V|-k$ and $|\mathcal{S}(k)\setminus \mathcal{R}(k)|=|V\setminus \mathcal{R}(k)|$ are satisfied or not. If they are not satisfied we can conclude that there is no such PSNE. Otherwise, we set the response of all the players in $V\setminus \mathcal{R}(k)$ as 0. Next we choose $|V|-k-|V\setminus \mathcal{R}(k)|$ players from $\mathcal{R}(k)\cap\mathcal{S}(k)$ and make their response as 0. Then we make responses of rest of the $k$ players as 1. Return the responses as PSNE.
\end{proof}


==> higher.tex <==
\section{Higher level proof ideas for the theorems}
\begin{theorem}
	The \psne problem is \NPC for sub-additive strict BNPG games even if the underlying graph is $3$-regular and the number of different utility functions is $2$. In particular, the \psne problem parameterized by (maximum degree, number of different utility functions) is \PNPH even for sub-additive strict BNPG games.
\end{theorem}
\textbf{Proof Idea:} We reduce from an instance of \tsat to the \psne problem for BNPG game. For every clause in \tsat instance we create a node for the \psne instance. Similarly for every literal we create a node for the \psne instance. Next we add the set of edges and define the best response functions in such a way that all clause nodes play $1$ in any PSNE and a set of literal nodes play $1$ in a PSNE iff and only there is satisfying assignment where the same set of literal nodes is assigned TRUE. This would complete the reduction 
\begin{theorem}
	The \psne problem parameterized by $k_1$ is \WTH even for the fully homogeneous BNPG game. Also the \psne problem parameretized by $k_0$ is \WTH even for the fully homogeneous BNPG game.
\end{theorem}
\textbf{Proof Idea:} We reduce from an instance of \ds to the \psne problem for BNPG game. We consider the underlying graph \GG for the \psne problem to be identical to the graph of \ds instance. We first define the best response functions in such a way that the set of $k$ vertices play 1 in PSNE if and only if the same set of $k$ vertices form a dominating set of \GG. This shows that the \psne problem for BNPG game parameterized by $k_1$ is \WTH. Similarly by appropriately defining the best response functions, we can show that the \psne problem for BNPG game parameterized by $k_0$ is \WTH
\begin{theorem}
	The \psne problem for the BNPG game parameterized by treewidth is \WOH.
\end{theorem}
\textbf{Proof idea:} To prove \WO-hardness, we reduce from \GFAC to \psne problem for BNPG game. For each vertex and edge in the graph $\GG$ associated with \GFAC instance, we add a node in the graph $\HH$ associated with \psne problem instance. On top of that we add some extra nodes and edges in \HH and appropriately define the best response functions of every player in \HH so that a set of nodes in \HH corresponding to a set \FF of edges belonging to \GG play $1$ in a PSNE if and only if \FF makes \GFAC an yes instance. 
\begin{theorem}
	\begin{enumerate}[(i)]
		\item The \psne problem for fully homogeneous BNPG games is \NPC even if the diameter of the graph is at most $4$.
		\item The \psne problem for fully homogeneous BNPG games is \WOH with respect to the parameter treewidth of the graph.
	\end{enumerate} 
\end{theorem}
\textbf{Proof idea:} We reduce from a heterogeneous BNPG game on \GG to a fully homogeneous game on \HH. In order to create \HH we take a copy of \GG, add some special set of nodes and some set of edges. We define the best response function in such a way that the nodes in \HH corresponding to nodes in \GG don't have their set of possible $n_v$ values overlapping with any other node in any PSNE for \HH. This allows us to make the nodes (excluding the special set of nodes which always play $1$ in PSNE) in \HH behave in the same way as the corresponding nodes in \GG if PSNE exists for any instance. This implies both instance are equivalent and the results in theorem follow.    
\begin{theorem}
	The \psne problem for fully homogeneous BNPG games is \NPC even if the maximum degree $\Delta$ of the graph is at most $9$.
\end{theorem}
\textbf{Proof idea:} Higher level idea is same as the previous Theorem. The only difference is that we add the special nodes in a way such that the maximum degree in the instance of fully homogeneous BNPG game is upper bounded by $9$.
\begin{theorem}
	There is an algorithm for the \psne problem for strict BNPG games which runs in time $\OO^*(2^\vc)$.
\end{theorem}
\textbf{Proof idea:} For every possible set of response of players in the vertex of the instance graph \GG, there is only one best response for the players in the vertex. This is due to fact that we are looking at a strict BNPG game and the set of nodes not in vertex cover form an independent set. So we can brute force over all possible set of responses of players in the vertex of the instance graph \GG and check the existence of PSNE.
\begin{theorem}
There is an algorithm running in time $\OO^*(4^{d_1})$ for the \psne problem in BNPG games where $d_1$ is the circuit rank of the input graph. 
\end{theorem}
\textbf{Proof idea:}First we provide an algorithm for checking the existence of PSNE in a BNPG game on \GG where \GG is a connected graph. We find a minimum spanning tree \TT of \GG. Then we find those set of vertices \VV' whose degree in \GG is not equal to the degree in \TT. Let \SS be all possible set of responses of players in \VV'. Then for each $t\in\SS$, we check whether there is a PSNE of \TT in which set of responses of \VV' is $t$. The players' utility functions are suitably modified while finding a PSNE in \TT for each possible $t\in\SS$ so that there is a PSNE in \GG if and only if there is PSNE in \TT for atleast one tuple $t\in\SS$. Now if the original instance graph \GG' has more than one component there is a PSNE in \GG if and only if there is a PSNE in each and every component of \GG'  
\begin{theorem}
The problem of determining the existence of PSNE in a BNPG game(\GG(\VV,\EE),\UU) is solvable in time $4^{d_2}\cdot n^{O(1)}$ where \GG is a connected graph.
\end{theorem}
\textbf{Proof idea:} If the instance graph \GG has more than $1$ component, then we can directly brute force as in this case $d_2\geq n-1$. So we assume that \GG(\VV,\EE) is a connected graph. Then we find those set of vertices \VV' whose degree in \GG is not equal to $n-1$. Let $\GG[\VV\setminus\VV']$ be an induced graph of \GG on those vertices which have degree $n-1$. Let \SS be all possible set of responses of players in \VV'. Then for each $t\in\SS$, we find PSNEs (if it exists) of $\GG[\VV\setminus\VV']$ where exactly $k$ players play $1$, $\forall k \in \{0,\ldots,|\VV\setminus \VV'|\}$. The players' utility functions are suitably modified while finding a PSNE in $\GG[\VV\setminus\VV']$ for each possible $t\in\SS$ so that there is a PSNE in \GG if and only if there is a $t\in\SS$ and PSNE $(x_v^*)_{v\in \VV\setminus\VV'}$ in \HH such that $t\cup (x_v^*)_{v\in \VV\setminus\VV'}$ is a PSNE in \GG.

==> results_old.tex <==
\section{Contribution}

\begin{table}[!htbp]
	\centering
	\begin{tabular}{|c|c|}\hline
		\textbf{Parameters } & \textbf{Result in heterogeneous BNPG games}\\\hline\hline
		
		maximum degree & \PNPH~[\Cref{thm:deg}]\\\hline
		
		diameter & \PNPH~[\Cref{thm:dia}]\\\hline
		
		$d_1$[\Cref{def:d1}] & FPT[\Cref{thm:d1}]\\\hline
		$d_2$[\Cref{def:d1}] & FPT[\Cref{thm:d2}]\\\hline
		
		number of zeroes in PSNE & W[1]-Hard~[\Cref{thm:0}] \\\hline

		number of ones in PSNE & W[1]-Hard~[\Cref{thm:1}] \\\hline
		treewidth & W[1]-Hard~[\Cref{thm:tw}] \\\hline
		%number of players whose utility functions\\ are not convex & FPT[\Cref{thm:con}]\\\hline
		%reduction to DAG[incomplete]& ~[\Cref{thm:red_dag}]\\\hline\hline

		%\textbf{Problem under Assumption} & \textbf{Result} \\\hline\hline
		
		

		%best response of each player $i\in[n]$ is 0 for\\ $n_i \leq n_{0_i}$ and 1 otherwise. & Polynomial Time Algorithm ~[\Cref{thm:0->1}]\\\hline

		
	\end{tabular}
	\caption{Summary of results.}
\end{table}
\section{Results}
W.l.o.g we assume that the graph $\mathcal{G}(\VV,\EE)$ of a BNPG game in this section is connected
\begin{theorem} \label{thm:deg}
Determining the existence of PSNE in a BNPG game on a graph $\mathcal{G}$ is NP-complete even if the maximum out degree $\Delta$ of graph $\mathcal{G}$ is 3.
\end{theorem}

\begin{proof}
	The  problem of determining PSNE in a BNPG game clearly belongs to \NP. To show its \NP-hardness, we reduce from \tsat. Let $(\XX=\{x_i:{i\in[n]}\}, \CC=\{C_j: j\in[m]\})$ be an arbitrary instance of \tsat. We define a function $f:\{x_i,\bar{x}_i: i\in[n]\}\longrightarrow\{a_i,\bar{a}_i: i\in[n]\}$ as $f(x_i)=a_i$ and $f(\bar{x}_i)=\bar{a}_i$ for $i\in[n]$. We consider the following instance $(\GG=(\VV,\EE))$.
	\begin{align*}
		\VV &= \{a_i, \bar{a}_i: i\in[n]\} \cup \{y_j: j\in[m]\}\\
		\EE &= \{(y_j,f(l_1)), (y_j,f(l_2)), (y_j,f(l_3)): C_j=(l_1\vee l_2\vee l_3), j\in[m]\}\\
		&\cup \{(a_i,\bar{a}_i): i\in[n]
	\end{align*}
	We observe that both the degree of every vertex in \GG is at $3$. Let us now define the best response policy for all the vertices in the graph $\mathcal{H}$. Let $n_{v}$ denote the number of neighbours of vertex $v\in\mathcal{V}$ who choose $1$ as their response. Let $z_{v}$ denote the best response of a vertex $v\in\mathcal{V}$ for a given value of $n_{v}$.

 $\forall j\in[m],z_{y_j}= \left\{ \begin{array}{rcl}
0 & \mbox{for} & n_{y_j}=0  \\ 
1 & \mbox{for} & n_{y_j}>0 
\end{array}\right.$

 $\forall j\in[n],z_{a_j}= \left\{ \begin{array}{rcl}
1& \mbox{for} & n_{a_j}\leq2  \\ 
0 & \mbox{for} & n_{a_j}=3 
\end{array}\right.$

 $\forall j\in[n],z_{\bar{a}_j}= \left\{ \begin{array}{rcl}
1& \mbox{for} & n_{\bar{a}_j}\leq2  \\ 
0 & \mbox{for} & n_{\bar{a}_j}=3 
\end{array}\right.$

We claim that BNPG game run of graph \GG has a PSNE if and only if \tsat instance is a \YES instance.
	
	Suppose the \tsat instance is a \YES instance. Let $g:\{x_i: i\in[n]\}\longrightarrow\{\true, \false\}$ be a satisfying assignment of the \tsat instance. Then in the instance of BNPG game on graph \GG let us consider the following response by the vertices in \VV:
\begin{itemize}
\item $\forall j\in[m],z_{y_j}=1$
\item $\forall i\in[n],z_{a_i}=1$ if and only if $g(x_i)=\true$
\item $\forall i\in[n],z_{\bar{a}_i}=0$ if and only if $g(x_i)=\true$
\end{itemize}
Now we argue that the above response forms a PSNE for the BNPG game.$\forall j\in[m]$, there is atleast one literal in clause $C_j$ which is always true. This implies that $\forall j\in[m]$, $n_{y_j}>0$. So, $\forall j\in[m]$, $y_j$ never deviates . For any $i\in[n]$, if $z_{a_i}=0$ then $z_{\bar{a}_i}=1$. Also $\forall j\in[m]$, $z_{y_j}=1$. This implies $n_{a_i}=3$ and $n_{\bar{a}_i}=2$. Hence $a_i,\bar{a}_i$ won't deviate if $z_{a_i}=0$. Similarly for any $i\in[n]$, if $z_{a_i}=1$ then $z_{\bar{a}_i}=0$. Also $\forall j\in[m]$, $z_{y_j}=1$.  This implies $n_{a_i}=2$ and $n_{\bar{a}_i}=3$. Hence $a_i,\bar{a}_i$ won't deviate if $z_{a_i}=1$.  Hence we have a PSNE.\\
	
	In the other direction, let there be PSNE for the BNPG game on \GG. First we show that for any such PSNE, $\forall j\in[m]$, $z_{y_j}=1$. We prove it using contradiction. Let us assume that $\exists k\in[m]$ such that $z_{y_k}=0$. Let the literals in clause $C_k$ be $l_1,l_2,l_3$. Then $z_{f(l_i)}=0,\forall i\in[3]$ otherwise $y_k$ will deviate. But then $f(l_1)$ will deviate to 1 as $n_{f(l_1)}\leq 2$. Hence there is no PSNE and therefore we have a contradiction. So if we have a PSNE then $\forall j\in[m]$, $z_{y_j}=1$. Now we show that in any PSNE, we have $z_{a_i}\neq z_{\bar{a}_i},\text{ }\forall i\in[n]$. We prove it using contradiction. First, let us assume that $\exists k_1\in[n]$ such that $z_{a_{k_1}}=z_{\bar{a}_{k_1}}=1$. As $\forall j\in[m]$, $z_{y_j}=1$, so $n_{a_{k_1}}=3$ and hence $a_{k_1}$ will deviate to 0. So we don't have a PSNE in this case. Now let us assume that $\exists k_2\in[n]$ such that $z_{a_{k_2}}=z_{\bar{a}_{k_2}}=0$. As $\forall j\in[m]$, $z_{y_j}=1$, so $n_{a_{k_2}}=2$ and hence $a_{k_2}$ will deviate to 1. So we don't have a PSNE even in this case and hence we have a contradiction. So in any PSNE, we have $z_{a_i}\neq z_{\bar{a}_i},\text{ }\forall i\in[n]$. Let $g:\{x_i: i\in[n]\}\longrightarrow\{\true, \false\}$ be an assignment of the \tsat instance such that $g(x_i)=\true$ if and only if $z_{a_i}=1$ in the PSNE. Hence $g$ is a satisfying assignment for the \tsat instance as $\forall j\in[m]$ $n_{y_j}>0$ otherwise $y_j$ will deviate to 0 and thus the \tsat instance is a \yes instance.

This concludes the proof of this theorem.

\end{proof}

\begin{corollary}
If the functions $g_i(.)$ is subadditive for $\forall i\in [n]$,still the problem of determining the existence of PSNE in a BNPG game on a graph $\mathcal{G}$ is NP-complete
\end{corollary}
\begin{proof}
In the \Cref{thm:deg}, for players in \GG we can define the utility function in the following way such that the functions $g_i(.)$ are subadditive:\\
$\forall j\in[m],\text{ }c_{y_j}=4,g_{y_j}(x)= \left\{ \begin{array}{rcl}
1000 & \mbox{if} & x=0  \\ 
1003 & \mbox{for} & x=1\\
 1008 & \mbox{for} & x=2\\
1013 & \mbox{for} & x=3\\
1018 & \mbox{for} & x=4
\end{array}\right.$\\
$\forall i\in[n],\text{ }c_{a_j}=c_{\bar{a}_j }=4,g_{a_j}(x)=g_{\bar{a}_j}(x)= \left\{ \begin{array}{rcl}
1000 & \mbox{if} & x=0  \\ 
1005 & \mbox{for} & x=1\\
 1010 & \mbox{for} & x=2\\
1015 & \mbox{for} & x=3\\
1018 & \mbox{for} & x=4
\end{array}\right.$
\end{proof}
\begin{lemma}\label{thm:dia}
Determining the existence of PSNE in a BNPG game on a graph $\mathcal{G}$ is NP-complete even if the diameter $d$ of graph $\mathcal{G}$ is atmost 2.
\end{lemma}
\begin{proof}
In Theorem 1 of \cite{yu2020computing}, the graph \HH created has a diameter of atmost 2. And since the problem of determining PSNE for the BNPG game on \HH is NP-complete according to Theorem 1 of \cite{yu2020computing}, we conclude that the existence of PSNE in a BNPG game on any graph $\mathcal{G}$ is NP-complete even if the diameter $d$ of graph $\mathcal{G}$ is atmost 2.
\end{proof}
\begin{observation}
The problem of determining the existence of PSNE in a BNPG game is $FPT$ with respect to the parameters $(\Delta,d)$
\end{observation}
\begin{proof}
In graph theory, the degree diameter problem is the problem of finding the largest possible graph G (in terms of the size of its vertex set V) of diameter $d$ such that the largest degree of any of the vertices in G is at most \Delta. The size of G is bounded above by the Moore bound which is $O(\Delta^d)$. Hence we can brute force in time $O(2^{O(\Delta^d)}\cdot O(\Delta^{d\cdot O(1)}))$ by checking every possible set of responses by the players and conclude whether there is any PSNE or not. 
\end{proof}
\begin{observation}
If the functions $g_i(.)$ is additive for $\forall i\in [n]$, the problem of determining the existence of PSNE in a BNPG game on a graph $\mathcal{G}$ is solvable in time $O(n)$
\end{observation}
\begin{definition}\label{def:d1}
Let the number of edges and number of vertices in graph $\mathcal{G}$ be $m$ and $n$ respectively. Then $d_{1}$ is defined to be $m-(n-1)$ and $d_2$ is defined to be $\frac{n(n-1)}{2}-m$. 
\end{definition}
\begin{theorem}\label{thm:d1}
The problem of determining the existence of PSNE in a BNPG game is solvable in time $4^{d_1}\cdot n^{O(1)}$
\end{theorem}
\begin{proof}
Given a graph \GG(\VV,\EE) on which we will be running the BNPG game, find the minimum spanning tree \TT (can be found in time $O(n^{O(1)})$).  Let $\EE'\subset\EE$ be the set of edges which are not part of \TT. Also by definition, $|\EE'|=d_1$. Let $\VV'\subseteq\VV$ be the set of vertices which are endpoints of atleast one edge in \EE'. This implies that $|\VV'|\leq 2d_1$. Let \VV'=$\{v_1,v_2,\ldots,v_l\}$ where $l\leq 2d_1$. Let the tuple $(x_{v_i})_{i\in [l]}$ denote the set of responses of players in \VV', where $x_{v_i}$ is the response of $v_i$. Let $\mathcal{S}$ be the set of all such possible tuples. Clearly $|\mathcal{S}|\leq2^{2d_1}$. For each $t\in \mathcal{S}$, we do the following:
\begin{enumerate}
\item For each $v\in\VV'$, let $n_v'$ be the number of neighbours of $v$ in \GG which are not neighbours in \TT and the response of such neighbours in the tuple $t$ is 1.   
\item Let us define functions $g'_v(.)$ such that $g'_v(x)=g_v(x)$ if $v\notin \VV'$ and $g'_v(x)=g_v(x+n_v')$ if $v\in\VV'$.
\item Run the fixed version of algorithm mentioned in Theorem 3 of \cite{yu2020computing} (for the fix please refer to \Cref{algo2:fix}) on \TT by considering the following constraints:
\begin{itemize}
\item Run the algorithms by considering the following utility function:
\begin{equation*}
U_v'(x_v,n_v)=g_v'(x_v+n_v)-c_ix_v
\end{equation*}
\item Before returning the table $T_Y$, remove a pair $(x_W,x_Y)$ from $T_Y$ if either $W\in\VV'$ and $x_W$ is not equal to the response of $W$ in $t$ or  $Y\in\VV'$ and $x_Y$ is not equal to the response of $Y$ in $t$.
\end{itemize}
 
If $\forall t\in \TT$ the modified algorithm above when ran on $t$ and \TT returns NO PSNE exists, then we have a NO instance otherwise we have a YES instance. The running time of this algorithm is clearly $4^{d_1}\cdot n^{O(1)}$

We now the present the proof idea for the correctness of the procedure metioned above. First we show that if we fix a tuple $t\in \mathcal{S}$ (by fixing we mean that the vertices in \VV' follow the responses in $t$), then there exists a PSNE in BNPG game on \GG if and only if there exists a PSNE in BNPG game on \TT with the modified utility functions.

Let $(x_v^*)_{v\in\VV}$ be the PSNE in BNPG game on \GG. Now we claim that $(x_v^*)_{v\in\VV}$ is also a PSNE in BNPG game on \TT with the modified utility functions. Let $n^\GG_v$ (resp.$n^\TT_v$)  denote the number of neighbours of $v$ in \GG (resp. \TT) whose response is 1. Clearly  $\forall v\in \VV'$ $n^\GG_v=n^\TT_v+n_v'$ and $\forall v\notin \VV'$ $n^\GG_v=n^\TT_v$. So $\forall v\notin \VV'$, $g'(n^\TT_v+1)-g'(n^\TT_v)=g(n^\GG_v+1)-g(n^\GG_v)$ and therefore $v$ won't deviate in \TT. Similarly $\forall v\in \VV'$, $g'(n^\TT_v+1)-g'(n^\TT_v)=g(n^\TT_v+n_v'+1)-g(n^\GG_v+n_v')=g(n^\GG_v+1)-g(n^\GG_v)$ and therefore $v$ won't deviate in \TT. Hence $(x_v^*)_{v\in\VV}$ is also a PSNE in BNPG game on \TT with the modified utility functions. In similar fashion we can show that if $(x_v^*)_{v\in\VV}$ is a PSNE in BNPG game on \TT with the modified utility functions then $(x_v^*)_{v\in\VV}$ is also a PSNE in BNPG game on \GG.

Given a tuple $t\in \TT$, we now argue that our procedure will correctly determine whether there is a PSNE in BNPG game on \TT or not.  The algorithms mentioned in Theorem 3 of \cite{yu2020computing} in general correctly determine whether there is a PSNE or not for a tree by indirectly searching over all the possible set of responses of the players. Now the only modification which we do is restricting the search to only those set of response such that players in \VV' follow the responses in $t$. Hence given a tuple $t \in \TT$ our procedure will correctly determine whether there is a PSNE in BNPG game on \TT. 

So if there is a PSNE in BNPG game on \GG, then there should exist a tuple $t$ such that there is a PSNE in BNPG game on \TT. Since we are searching over all tuples we will eventually hit the tuple $t$ and output the correct PSNE. Also if there is no PSNE in BNPG game on \GG, then $\forall t\in \mathcal{S}$,our modified algorithm when ran on $t$ and \TT returns NO PSNE exists and hence we correctly conclude it as NO instance. This concludes the proof of this theorem 
\end{enumerate}
\end{proof}
\begin{theorem}\label{thm:d2}
The problem of determining the existence of PSNE in a BNPG game on \GG(\VV,\EE) is solvable in time $4^{d_2}\cdot n^{O(1)}$
\end{theorem}
\begin{proof}
Let $\VV'=\{u|\exists v\in \VV\text{ such that }(u,v)\notin\EE,\forall u \in \VV\}$. Number of edges not in \EE is $d_2$, so $|\VV'|\leq 2d_2$. Let \HH be the induced subgraph of \GG on set of vertices  $\VV\setminus\VV'$. Clearly all the vertices in $\VV\setminus\VV'$ have a degree of $n-1$ and hence \HH is a complete graph. Let \VV'=$\{v_1,v_2,\ldots,v_l\}$ where $l\leq 2d_2$. Let the tuple $(x_{v_i})_{i\in [l]}$ denote the set of responses of players in \VV', where $x_{v_i}$ is the response of $v_i$. Let $\mathcal{S}$ be the set of all such possible tuples. Clearly $|\mathcal{S}|\leq2^{2d_2}$. For each $t\in \mathcal{S}$, we do the following:
\begin{enumerate}
\item Let $n_{v}^{t}$ denote the neighbours of $v$ in \VV' whose responses are 1 in the tuple $t$
\item Let $n_{\VV'}$ be the number of 1 in the tuple $t$.
\item $\forall v \in \VV\setminus \VV'$, let us define functions $g'_v(.)$ such that $g'_v(x)=g_v(x+n_{\VV'})$.
\item Run the algorithm mentioned in \Cref{prop2:fix} on \HH by considering the following utility function:
\begin{equation*}
U_v'(x_v,n_v)=g_v'(x_v+n_v)-c_ix_v
\end{equation*}
\item Let $\mathcal{K}_t=\{k|$ there is a PSNE where exactly $k$ players have their response as 1, $\forall k\in[n]\}$. Clearly this set can be computed in $n^{O(1)}$ time during the run of the algorithm in \Cref{prop2:fix}.
\item If $\exists k\in \mathcal{K}_t$ such that $\forall v\in \VV'$, $v$ won't deviate from it's response in $t$ given that $n_v=n_v^t+k$ then output "PSNE exists"
\end{enumerate}
If the above procedure ever returns PSNE exists then it's an YES instance otherwise it's a NO instance. The running time of this algorithm is clearly $4^{d_2}\cdot n^{O(1)}$\\


Clearly if $\exists t\in \mathcal{S}$ and $k\in \mathcal{K}_t$ such that Step 6 of the above the procedure is satisfied, then we surely have a PSNE for the game on \GG. PSNE is the responses of \VV' in $t$ and response of players in \HH such that the number of responses which are 1 in \HH is $k$. Let $n_{v}^{\HH}$ denote the neighbours of $v$ in the graph \HH whose responses are 1.  None of the vertices in $\VV'$ deviate due to the choice of $k$ and the fact that $n_v=n_v^t+k$ (as $n_{v}^{\HH}$ $\forall v \in \VV'$) . Also for all the vertices $v$ in \HH, $g'_v(n_v^{\HH}+1)-g'_v(n_v^{\HH})=g_v(n_v+1)-g_v(n_v)$ (as $n_v^{\HH}+n_{\VV'}=n_v$). Hence none of the vertices in \HH will deviate hence we have a PSNE in \GG.\\

Now suppose that we have a PSNE in \GG. Let $t\in mathcal{S}$ be the tuple such that responses of players \VV' in PSNE matches with that of $t$. Let the number of vertices in \HH whose response is 1 in this PSNE be $k$. For all the vertices $v$ in \HH, $g'_v(n_v^{\HH}+1)-g'_v(n_v^{\HH})=g_v(n_v+1)-g_v(n_v)$ (as $n_v^{\HH}+n_{\VV'}=n_v$). Hence the response of the players in \HH for a PSNE for BNPG game on \HH too. So $k\in \mathcal{K}_t$. Also since none of the players in $\VV'$ deviate and also we have $n_v=n_v^t+k$ , so the condition in Step 6 of our procedure is satisfied and hence we output "PSNE exists".\\

This concludes the proof of the theorem. 
\end{proof}
\begin{definition}
(Vertex Deletion to Regular Subgraph (VDRS)) Given a graph $G$ and two non-negative integers $k$ and $r$, is there an $r$-regular subgraph of $G$ obtainable by at most $k$ vertex deletions.
\end{definition}
\begin{lemma}
VDRS is W[1]-Hard with respect to the parameter $k$.
\end{lemma}
\begin{theorem}\label{thm:0}
The problem of determining the existence of PSNE with atmost $k$ zeroes chosen by the players in a BNPG game is $W[1]-Hard$ with respect to the parameter $k$
\end{theorem}
\begin{proof}
To prove $W[1]-Hardness$, we reduce from VDRS to BNPG game. Let $G(V,E)$ and two non-negative integers $k$ and $r$ be an arbitrary instance of VDRS. Now using this instance of VDRS we create an instance of BNPG Game. Let \GG(\VV,\EE) be a graph such that \VV=$V$ and \EE=$E$. \\\\
Let us now define the best response policy for all the vertices in the graph $\mathcal{G}$. Let $n_{v}$ denote the number of neighbours of vertex $v\in\mathcal{V}$ who choose $1$ as their response. Let $x_{v}$ denote the best response of a vertex $v\in\mathcal{V}$ for a given value of $n_{v}$.\\
$x_{v}= \left\{ \begin{array}{rcl}
1 & \mbox{for} & n_{v}=r  \\ 
0 & \mbox{for} & n_{v}\neq r 
\end{array}\right.$
We claim that BNPG game run of graph $\mathcal{G}$ has a PSNE with atmost $k$ zeroes if and only if $VDRS$ is an YES instance. 

In one direction, let VDRS be an YES instance. Let $V'$ be the set of atmost $k$ vertices which get deleted so that $V\setminus V'$ is a $r$-regular subgraph in $G$. Note that $|V\setminus V'|\geq r+1$. Now consider the following responses for players in graph \GG. For $\forall v \in V'$ let the response be 0 and $\forall v \in V\setminus V'$ let the response be 1. Clearly any player $v$ in $V'$ won'r deviate as $n_v \geq r+1$. Any player $v$ in $V\setminus V'$ won't deviate as $n_v=r$. Hence BNPG game run of graph $\mathcal{G}$ has a PSNE with atmost $k$ zeroes. 

In the other direction, let us have a PSNE for the BNPG game with atmost $k$ ones. Let $\VV'$ be the set of players are responses are 1. Clearly then $\VV \setminus \VV'$ forms a $r$-regular subgraph otherwise the players would deviate as in this case for some vertex $v\in \VV \setminus \VV'$, $n_v$ would not be equal to $d_v-r$. This implies VDRS is an YES instance as we can delete the set of vertices $\VV'$ from $G$ and get a $r$-regular subgraph. 


This concludes the proof of the theorem.
\end{proof}
\begin{theorem}\label{thm:1}
The problem of determining the existence of PSNE with atmost $k$ ones chosen by the players in a BNPG game is $W[1]-Hard$ with respect to the parameter $k$
\end{theorem}
\begin{proof}
To prove $W[1]-Hardness$, we reduce from VDRS to BNPG game. Let $G(V,E)$ and two non-negative integers $k$ and $r$ be an arbitrary instance of VDRS. Now using this instance of VDRS we create an instance of BNPG Game. Let \GG(\VV,\EE) be a graph such that \VV=$V$ and \EE=$E$. \\\\
Let us now define the best response policy for all the vertices in the graph $\mathcal{G}$. Let $n_{v}$ denote the number of neighbours of vertex $v\in\mathcal{V}$ who choose $1$ as their response. Let $x_{v}$ denote the best response of a vertex $v\in\mathcal{V}$ for a given value of $n_{v}$. Let $d_v$ be the degree of vertex $v$.\\
$x_{v}= \left\{ \begin{array}{rcl}
1 & \mbox{for} & n_{v}=d_v-r  \\ 
0 & \mbox{for} & n_{v}\neq d_v-r 
\end{array}\right.$
We claim that BNPG game run of graph $\mathcal{G}$ has a PSNE with atmost $k$ ones if and only if $VDRS$ is an YES instance.

In one direction, let VDRS be an YES instance. Let $V'$ be the set of atmost $k$ vertices which get deleted so that $V\setminus V'$ is a $r$-regular subgraph in $G$. Note that $|V\setminus V'|\geq r+1$. Now consider the following responses for players in graph \GG. For $\forall v \in V'$ let the response be 1 and $\forall v \in V\setminus V'$ let the response be 0. Clearly any player $v$ in $V'$ won't deviate as $n_v \leq d_v-(r+1)$. Any player $v$ in $V\setminus V'$ won't deviate as $n_v=d_v-r$. Hence BNPG game run of graph $\mathcal{G}$ has a PSNE with atmost $k$ ones.  

In the other direction, let us have a PSNE for the BNPG game with atmost $k$ ones. Let $\VV'$ be the set of players are responses are 1. Clearly then $\VV \setminus \VV'$ forms a $r$-regular subgraph otherwise the players would deviate as in this case for some vertex $v\in \VV \setminus \VV'$, $n_v$ would not be equal to $d_v-r$. This implies VDRS is an YES instance as we can delete the set of vertices $\VV'$ from $G$ and get a $r$-regular subgraph. 
\end{proof}
\begin{definition}
(GENERAL FACTOR). Given a graph $G$ and for each vertex $v$ of $G$ a set $K(v)\subseteq\{0,...,d(v)\}$, is there a subset $F\subseteq E(G)$ such that for each vertex $v\in V(G)$ the number of edges in $F$ incident with $v$ is an element of $K(v)$? 
\end{definition}
\begin{lemma}
GENERAL FACTOR is $W[1]-Hard$ when parameterized by the treewidth of the instance graph.
\end{lemma}
\begin{theorem}\label{thm:tw}
The problem of determining the existence of PSNE in a BNPG game is $W[1]-Hard$ with respect to the parameter treewidth.
\end{theorem}
\begin{proof}
To prove $W[1]-Hardness$, we reduce from GENERAL FACTOR to BNPG game. Let ($G(V,E)$ and $\forall v\in V, K(v)\subseteq\{0,...,d(v)\}$) be an arbitrary instance of GENERAL FACTOR.
For the remainder of the proof, let V=$\{v_1,v_2,\ldots,v_n\}$. Now using this instance of GENERAL FACTOR we create an instance of BNPG Game. Let us construct a graph $\mathcal{H}=(\mathcal{V,E})$ where $\mathcal{V}=V_1\cup V_2 \cup V_3 \cup \{d_1\} \cup \{d_2\}$. $V_1=V$. For all edges $(u,v) \in E$ we create a node $a_{uv}$ and add it to the set $V_2$. We add $n+1$ nodes $\{v_1',v_2',\ldots,v_{n+1}'\}$ to the set $V_3$. $\forall a_{uv}\in V_2$, $(a_{uv},u)\in\mathcal{E}$ and $(a_{uv},v)\in\mathcal{E}$.  $\forall i\in[n],(v_i',v_i)\in\mathcal{E}$ and $(d_1,v_i')\in\mathcal{E}$. $\forall i\in[n],(v_i,d_2)\in\mathcal{E}$. Also,  $(d_1,v_{n+1}')\in\mathcal{E}$ and $(d_2,v_{n+1})\in\mathcal{E}$. This completes the construction of graph $\mathcal{H}$.  In the nice tree decomposition of $G$ we can add the nodes $d_1,d_2$ to each and every bag. This increases the treewidth by 2. $\forall u\in V_2\cup V_3$ whenever the neighbours of $u$ in graph $\mathcal{H}$ are in the same bag $X_t$ for the first time in the tree decomposition if we started searching from the root then we can add two bags $X_{t_1}$ and $X_{t_2}$ between $X_t$ and its child such that $X_t$ is parent of $X_{t_1}$ and $X_{t_1}$  is parent of $X_{t_2}$. $X_{t_1}=X_{t_1}\cup\{u\}$ and $X_{t_2}=X_t$. This increases the treewidth by 1. So if graph $G$ has treewidth $k$ then graph $\mathcal{H}$ has treewidth of atmost $k+3$.   \\ 
\\
Let us now define the best response policy for all the vertices in the graph $\mathcal{H}$. Let $n_{v}$ denote the number of neighbours of vertex $v\in\mathcal{V}$ who choose $1$ as their response. Let $x_{v}$ denote the best response of a vertex $v\in\mathcal{V}$ for a given value of $n_{v}$.

$ x_{d_1}= \left\{ \begin{array}{rcl}
0 & \mbox{for} & n_{d_1}=n+1  \\ 
1 & \mbox{for} & n_{d_1}=n \\
0 & \mbox{for} & 1\leq n_{d_1} < n\\
1 & \mbox{for} & n_{d_1}=0
\end{array}\right.$

 $x_{d_2}= \left\{ \begin{array}{rcl}
1 & \mbox{for} & n_{d_2}=0  \\ 
0 & \mbox{for} & n_{d_2}>0 
\end{array}\right.$

$ \forall u\in V_2,x_{u}= \left\{ \begin{array}{rcl}
0,1 & \mbox{for} & n_{u}\leq2 
\end{array}\right.$

$ \forall u\in V_1,x_{u}= \left\{ \begin{array}{rcl}
1 & \mbox{for} & n_{u}-1\in K(u)  \\ 
0 & \mbox{for} & otherwise
\end{array}\right.$

$ \forall u\in V_3,x_{u}= \left\{ \begin{array}{rcl}
1 & \mbox{for} & n_{u}=2  \\ 
0 & \mbox{for} & n_{u}<2 
\end{array}\right.$

We claim that BNPG game run of graph $\mathcal{H}$ has a PSNE if and only if there is a subset $F\subseteq E(G)$ such that for each vertex $v\in V(G)$ the number of edges in $F$ incident with $v$ is an element of $K(v)$. 

In one direction, let there exist a subset $F\subseteq E(G)$ which makes GENERAL FACTOR a YES instance. Then in the instance of BNPG game on graph $\mathcal{H}$ let us consider the following response by the vertices in $\mathcal{V}$:
\begin{itemize}
\item $x_{d_1}=1$
\item $\forall i\in[n],x_{v_i'}=1$
\item $x_{v_{n+1}'}=0$
\item $\forall i \in [n],x_{v_i}=1$
\item $x_{d_2}=0$
\item $ \forall a_{uv}\in V_2,x_{a_{uv}}= \left\{ \begin{array}{rcl}
1 & \mbox{if} & (u,v)\in F  \\ 
0 & \mbox{otherwise}  
\end{array}\right.$
\end{itemize}
Now we argue that the above response forms a PSNE for the BNPG game. Clearly no node in $V_2$ deviates because of the way its best response has been defined.  $d_1$ won't deviate as $n_{d_1}=n$. $\forall i\in[n],v_i'$ won't deviate as $n_{v_i'}=2$. $v_{n+1}'$ won't deviate as $n_{v_{n+1}'}=1$. $d_2$ won't deviate as $n_{d_2}>0$. $\forall i \in [n],v_i$ won't deviate as $n_{v_i}-1\in K(v_i)$. Hence we have a PSNE.\\
\\
In other direction, let there exist a PSNE for the BNPG Game on graph $\mathcal{H}$. If the responses of the players in the PSNE are such that  $x_{d_1}=1$, $\forall i\in[n]$ $x_{v_i'}=1$, $x_{v_{n+1}'}=0$, $\forall i \in [n]$ $x_{v_i}=1$, $x_{d_2}=0$ then the set $F=\{(u,v)|x_{a_{uv}}=1, a_{uv}\in V_2\}$ makes GENERAL FACTOR a YES instance as for each $v\in V_1$ , $n_{v}-1\in K(v)$ which implies number of edges in $F$ incident on $v$ in GENERAL FACTOR instance is an element of $K(v)$.\\
\\
Now we argue that any PSNE for the BNPG Game on graph $\mathcal{H}$  should have $x_{d_1}=1$, $\forall i\in[n]$ $x_{v_i'}=1$, $x_{v_{n+1}'}=0$, $\forall i \in [n]$ $x_{v_i}=1$, $x_{d_2}=0$. Let us assume that there is a PSNE which is not of the above form. Then we have the following possibilities:
\begin{enumerate}
\item ($\forall i \in [n]$ $x_{v_i}=1$). We must have $x_{d_2}=0$ so that $d_2$ doesn't deviate. This would imply that $x_{v_{n+1}'}=0$. In order for $d_1$ to not deviate we have two subcases.
\begin{itemize}
\item ($x_{d_1}=1$,$\forall i\in[n]$ $x_{v_i'}=0$ ). Here $v_{i'}'$ will then deviate to $1$ where $i'\in[n]$. Hence no PSNE is possible in this subcase.
\item ($x_{d_1}=0$, $\exists k_1,k_2\in [n]$ such that $x_{v_{k_1}'}=1$ and $x_{v_{k_2}'}=0$  ). No PSNE is possible as $v_{k_1}'$ will deviate to 0.
\end{itemize}
\item ($\exists k_1,k_2\in [n]$ such that $x_{v_{k_1}}=1$ and $x_{v_{k_2}}=0$ ). We must have $x_{d_2}=0$ so that $d_2$ doesn't deviate. This would imply that $x_{v_{n+1}'}=0$. Also $x_{v_{k_2}'}=0$ as $n_{v_{k_2}'}\leq1$. In order for $d_1$ to not deviate we have two subcases. 
\begin{itemize}
\item ($x_{d_1}=1$,$\forall i\in[n]$ $x_{v_i'}=0$). Here $v_{k_1}'$ will deviate to 1 and hence PSNE is not possible in this subcase.
\item ($x_{d_2}=0$,$\exists i\in[n]$ such that $x_{v_i'}=1$). Here $v_i'$ will deviate to 0 as $n_{v_i'}\leq1$ and hence PSNE is not possible in this subcase.
\end{itemize}
\item ($\forall i \in [n]$ $x_{v_i}=0$). $\forall i\in[n]$ we must have $x_{v_i'}=0$ so that $v_i'$ doesn't deviate. We have 6 subcases.
\begin{itemize}
\item $(x_{d_1}=0,x_{v_{n+1}'}=0).$ Here $d_1$ deviates to 1 as $n_{d_1}=0$ and hence PSNE is not possible in this subcase.
\item $(x_{d_1}=0,x_{v_{n+1}'}=1).$ Here $v_{n+1}'$ deviates to 0 as $n_{v_i'}\leq1$ and hence PSNE is not possible in this subcase.
\item $(x_{d_1}=1,x_{v_{n+1}'}=0,x_{d_2}=0).$ Here $d_2$ deviates to 1 as $n_{d_2}=0$ and hence PSNE is not possible in this subcase.
\item $(x_{d_1}=1,x_{v_{n+1}'}=0,x_{d_2}=1).$ Here $v_{n+1}'$ deviates to 1 as $n_{v_i'}=2$ and hence PSNE is not possible in this subcase.
\item $(x_{d_1}=1,x_{v_{n+1}'}=1,x_{d_2}=0).$Here $v_{n+1}'$ deviates to 0 as $n_{v_i'}=1$ and hence PSNE is not possible in this subcase.
\item $(x_{d_1}=1,x_{v_{n+1}'}=1,x_{d_2}=1).$Here $d_2$ deviates to 0 as $n_{d_2}>0$ and hence PSNE is not possible in this subcase.
\end{itemize}
\end{enumerate}

Since none of possibilities give us a PSNE, therefore our initial assumption was incorrect. Therefore if BNPG game is a YES instance then GENERAL FACTOR is also a YES instance. This concludes the proof of this Theorem. 
\end{proof}
\begin{figure}[h]

\centering
\includegraphics[width=0.5\textwidth]{9}
\caption{General Factor problem instance $G(V,E)$}
\end{figure}
\begin{figure}[h]

\centering
\includegraphics[width=0.5\textwidth]{10}
\caption{Reduction to BNPG game. Black vertices belong to $V_1$, yellow vertices belong to $V_2$, blue vertices belong to $V_3$, red node is $d_1$ and green node is $d_2$}
\end{figure}



\subsection{Problems left to be solved}
\begin{itemize}
\item The problem of determining the existence of PSNE in a homogeneous or fully homogeneous BNPG games with respect to parameters like treewidth, maximum degree .
\item Algorithm to find MSNE
\item Consider other utility functions such that best response is 1 for $n_i \leq n_0$ and 0 otherwise.
\item Decide whether $2^n$ is the best complexity or not
\item Fix Theorem 8 in \cite{yu2020computing}
\item Check if there is a polynomial time algorithm to find the all the PSNE of BNPG game if the best response of each player $i\in[n]$ is 0 for $n_i \leq n_{0_i}$ and 1 otherwise.
\item In an instance of BNPG game, let $t$ be the number of players whose utility function isn't convex. FInd FPT w.r.t $t$.
\end{itemize}

==> thm3.tex <==
\section{Theorem 3 and 4 rewritten}
\begin{definition}\label{def:d1}
Let the number of edges and number of vertices in a connected graph $\mathcal{G}$ be $m$ and $n$ respectively. Then $d_{1}$( circuit rank ) is defined to be $m-n+c$ ($c$ is the number of connected components in the graph) and $d_2$( distance from complete graph ) is defined to be $\frac{n(n-1)}{2}-m$. 
\end{definition}
\begin{theorem}\label{thm:d1}
The problem of determining the existence of PSNE in a BNPG game(\GG(\VV,\EE),\UU) is solvable in time $4^{d_1}\cdot n^{O(1)}$.
\end{theorem}
\begin{proof}
Let the graph \GG have $c$ connected components namely, $\GG_1,\ldots,\GG_c$. First we try to determine the existence of PSNE in each connected components separately. Consider a connected component $\GG_i(\VV_i,\EE_i)$ and find the minimum spanning tree $\TT_i$ (can be found in time $O(n^{O(1)})$).  Let $\EE_i'\subset\EE_i$ be the set of edges which are not part of $\TT_i$. Let $|\EE'|=d_1^i$. Let $\VV_i'\subseteq\VV_i$ be the set of vertices which are endpoints of atleast one edge in $\EE_i'$. This implies that $|\VV_i'|\leq 2d_1^i$. Let $\VV_i'$=$\{v_1^i,v_2^i,\ldots,v_l^i\}$ where $l\leq 2d_1^i$. Let the tuple $(x_{v_j^i})_{j\in [l]}$ denote the set of responses of players in $\VV_i'$, where $x_{v_j^i}$ is the response of $v_j^i$. Let $\SS_i$ be the set of all such possible tuples. Clearly $|\mathcal{S}_i|\leq2^{2d_1^i}$. For each $t\in \mathcal{S}_i$, we do the following:
\begin{enumerate}
\item For each $v\in\VV_i'$, let $n_v'$ be the number of neighbours of $v$ in $\GG_i$ which are not neighbours in $\TT_i$ and the response of such neighbours in the tuple $t$ is 1.   
\item Let us define functions $g'_v(.)$ such that $g'_v(x)=g_v(x)$ if $v\notin \VV_i'$ and $g'_v(x)=g_v(x+n_v')$ if $v\in\VV_i'$.
\item Run the fixed version of algorithms mentioned in Theorem 3 of \cite{yu2020computing} (for the theorem and algorithms please refer to \Cref{appendix:treePSNE} and for the fix please refer to \Cref{algo2:fix}) on $\TT_i$ by considering the following constraints:
\begin{itemize}
\item Run the algorithms by considering the following utility function:
\begin{equation*}
U_v'(x_v,n_v)=g_v'(x_v+n_v)-c_ix_v
\end{equation*}
\item Before returning the table $T_Y$, remove a pair $(x_W,x_Y)$ from $T_Y$ if either $W\in\VV'$ and $x_W$ is not equal to the response of $W$ in $t$ or  $Y\in\VV_i'$ and $x_Y$ is not equal to the response of $Y$ in $t$.
\end{itemize}
 
If $\forall t\in \TT_i$ the modified algorithm above when ran on $t$ and $\TT_i$ returns NO PSNE exists, then we have a NO instance. Else return YES instance for $\GG_i$. The running time of the above procedure on $\GG_i$ is clearly $4^{d_1^i}\cdot n^{O(1)}$

We now the present the proof idea for the fact that the above procedure correctly determines whether there is a PSNE in $\GG_i$ or not. First we show that if we fix a tuple $t\in \mathcal{S}_i$ (by fixing we mean that the vertices in $\VV_i'$ follow the responses in $t$), then there exists a PSNE in BNPG game on $\GG_i$ if and only if there exists a PSNE in BNPG game on $\TT_i$ with the modified utility functions.

Let $(x_v^*)_{v\in\VV}$ be the PSNE in BNPG game on $\GG_i$. Now we claim that $(x_v^*)_{v\in\VV_i}$ is also a PSNE in BNPG game on $\TT_i$ with the modified utility functions. Let $n^{\GG_i}_v$ (resp.$n^{\TT_i}_v$)  denote the number of neighbours of $v$ in $\GG_i$ (resp. $\TT_i$) whose response is 1. Clearly  $\forall v\in \VV_i'$ $n^{\GG_i}_v=n^{\TT_i}_v+n_v'$ and $\forall v\notin \VV_i'$ $n^{\GG_i}_v=n^{\TT_i}_v$. So $\forall v\notin \VV_i'$, $g'(n^{\TT_i}_v+1)-g'(n^{\TT_i}_v)=g(n^{\GG_i}_v+1)-g(n^{\GG_i}_v)$ and therefore $v$ won't deviate in $\TT_i$. Similarly $\forall v\in \VV_i'$, $g'(n^{\TT_i}_v+1)-g'(n^{\TT_i}_v)=g(n^{\TT_i}_v+n_v'+1)-g(n^{\GG_i}_v+n_v')=g(n^{\GG_i}_v+1)-g(n^{\GG_i}_v)$ and therefore $v$ won't deviate in $\TT_i$. Hence $(x_v^*)_{v\in\VV}$ is also a PSNE in BNPG game on $\TT_i$ with the modified utility functions. In similar fashion we can show that if $(x_v^*)_{v\in\VV_i}$ is a PSNE in BNPG game on $\TT_i$ with the modified utility functions then $(x_v^*)_{v\in\VV_i}$ is also a PSNE in BNPG game on $\GG_i$.

Given a tuple $t\in \SS_i$, we now argue that our procedure will correctly determine whether there is a PSNE in BNPG game on $\TT_i$ or not.  The algorithms mentioned in Theorem 3 of \cite{yu2020computing} in general correctly determine whether there is a PSNE or not for a tree by indirectly searching over all the possible set of responses of the players. Now the only modification which we do is restricting the search to only those set of response such that players in $\VV_i'$ follow the responses in $t$. Hence given a tuple $t \in \SS_i$ our procedure will correctly determine whether there is a PSNE in BNPG game on $\TT_i$. 

So if there is a PSNE in BNPG game on $\GG_i$, then there should exist a tuple $t$ such that there is a PSNE in BNPG game on $\TT_i$. Since we are searching over all tuples we will eventually hit the tuple $t$ and output the correct PSNE. Also if there is no PSNE in BNPG game on $\GG_i$, then $\forall t\in \mathcal{S}$,our modified algorithm when ran on $t$ and $\TT_i$ returns NO PSNE exists and hence we correctly conclude it as NO instance. 

Repeat the above procedure for each and every component in \GG. The total running time is $4^{\sum_{i=1}^{c}d_1^i}\cdot n^{O(1)}=4^{d_1}\cdot n^{O(1)}$. If for any component in \GG we get that it is a NO instance then we output BNPG game on \GG is NO instance otherwise we output BNPG game on \GG is YES instance. Correctness arises from the fact that there is a PSNE for BNPG game on \GG if and only if $\i \in [c]$ there is a PSNE for BNPG game on $\GG_i$
\end{enumerate}
\end{proof}
\begin{theorem}\label{thm:d2}
The problem of determining the existence of PSNE in a BNPG game(\GG(\VV,\EE),\UU) is solvable in time $4^{d_2}\cdot n^{O(1)}$ where \GG is a connected graph.
\end{theorem}
\begin{proof}
If \GG has more than one connected component then $d_2\geq n-1$ (this arises from the fact if a graph \GG has more than one connected component then maximum number of edges in \GG is (n-1)(n-2)/2), then we can directly brute force over all possible responses of the players in \GG and check whether there is any PSNE or not. The running time is $2^n\cdot n^{O(1)}\leq 4^{d_2}\cdot n^{O(1)}$. So for the rest of the proof we assume that \GG is connected. \\
Let $\VV'=\{u|\exists v\in \VV\text{ such that }(u,v)\notin\EE,\forall u \in \VV\}$. Number of edges not in \EE is $d_2$, so $|\VV'|\leq 2d_2$. Let \HH be the induced subgraph of \GG on set of vertices  $\VV\setminus\VV'$. Clearly all the vertices in $\VV\setminus\VV'$ have a degree of $n-1$ and hence \HH is a complete graph. Let \VV'=$\{v_1,v_2,\ldots,v_l\}$ where $l\leq 2d_2$. Let the tuple $(x_{v_i})_{i\in [l]}$ denote the set of responses of players in \VV', where $x_{v_i}$ is the response of $v_i$. Let $\mathcal{S}$ be the set of all such possible tuples. Clearly $|\mathcal{S}|\leq2^{2d_2}$. For each $t\in \mathcal{S}$, we do the following:
\begin{enumerate}
\item Let $n_{v}^{t}$ denote the neighbours of $v$ in \VV' whose responses are 1 in the tuple $t$
\item Let $n_{\VV'}$ be the number of 1 in the tuple $t$.
\item $\forall v \in \VV\setminus \VV'$, let us define functions $g'_v(.)$ such that $g'_v(x)=g_v(x+n_{\VV'})$.
\item Run the algorithm mentioned in \Cref{prop2:fix} on \HH by considering the following utility function:
\begin{equation*}
U_v'(x_v,n_v)=g_v'(x_v+n_v)-c_ix_v
\end{equation*}
\item Let $\mathcal{K}_t=\{k|$ there is a PSNE where exactly $k$ players have their response as 1, $\forall k\in[n]\}$. Clearly this set can be computed in $n^{O(1)}$ time during the run of the algorithm in \Cref{prop2:fix}.
\item If $\exists k\in \mathcal{K}_t$ such that $\forall v\in \VV'$, $v$ won't deviate from it's response in $t$ given that $n_v=n_v^t+k$ then output "PSNE exists"
\end{enumerate}
If the above procedure ever returns PSNE exists then it's an YES instance otherwise it's a NO instance. The running time of this algorithm is clearly $4^{d_2}\cdot n^{O(1)}$


Clearly if $\exists t\in \mathcal{S}$ and $k\in \mathcal{K}_t$ such that Step 6 of the above the procedure is satisfied, then we surely have a PSNE for the game on \GG. PSNE is the responses of \VV' in $t$ and response of players in \HH such that the number of responses which are 1 in \HH is $k$. Let $n_{v}^{\HH}$ denote the neighbours of $v$ in the graph \HH whose responses are 1.  None of the vertices in $\VV'$ deviate due to the choice of $k$ and the fact that $n_v=n_v^t+k$ (as $n_{v}^{\HH}$ $\forall v \in \VV'$) . Also for all the vertices $v$ in \HH, $g'_v(n_v^{\HH}+1)-g'_v(n_v^{\HH})=g_v(n_v+1)-g_v(n_v)$ (as $n_v^{\HH}+n_{\VV'}=n_v$). Hence none of the vertices in \HH will deviate hence we have a PSNE in \GG.

Now suppose that we have a PSNE in \GG. Let $t\in \mathcal{S}$ be the tuple such that responses of players \VV' in PSNE matches with that of $t$. Let the number of vertices in \HH whose response is 1 in this PSNE be $k$. For all the vertices $v$ in \HH, $g'_v(n_v^{\HH}+1)-g'_v(n_v^{\HH})=g_v(n_v+1)-g_v(n_v)$ (as $n_v^{\HH}+n_{\VV'}=n_v$). Hence the response of the players in \HH for a PSNE for BNPG game on \HH too. So $k\in \mathcal{K}_t$. Also since none of the players in $\VV'$ deviate and also we have $n_v=n_v^t+k$ , so the condition in Step 6 of our procedure is satisfied and hence we output "PSNE exists". This concludes the proof of the theorem. 
\end{proof}



